Personalized Recommendations in EdTech: Evidence from a Randomized Controlled Trial

We study the impact of personalized content recommendations on the usage of an educational app for children. In a randomized controlled trial, we show that the introduction of personalized recommendations increases the consumption of content in the personalized section of the app by approximately 60%. We further show that the overall app usage increases by 14%, compared to the baseline system where human content editors select stories for all students at a given grade level. The magnitude of individual gains from personalized content increases with the amount of data available about a student and with preferences for niche content: heavy users with long histories of content interactions who prefer niche content benefit more than infrequent, newer users who like popular content. To facilitate the move to personalized recommendation systems from a simpler system, we describe how we make important design decisions, such as comparing alternative models using offline metrics and choosing the right target audience.

==> sections/off_policy_section.tex <==
\section{Off-policy evaluation}\label{off_policy_section}

On-policy evaluation using a randomized experiment provides a simple and powerful framework to evaluate the impact of an introduction of a recommendation system on engagement. However, the number of alternative systems that can be evaluated in this way is limited by the number of users available and, thus, power in the experiment. Additionally, a concern for user experience might constrain the scope of evaluated systems. Therefore, an off-policy evaluation is a useful alternative.

In this section, we use off-policy evaluation to answer three questions: (i) Is a doubly-robust off-policy estimator a reliable estimator of mean \emph{Story Engagement}, and can we use it in place of a randomized experiment?  (ii) Would a popularity-based recommendation system bring similar gains to those from the personalized system; and (iii) Do the gains due to the new recommendation system stem from the algorithm being better at picking top stories or due to personalization? We use pre-experimental, experimental, and post-experimental data for the analysis in this section. This lets us exploit data availability under multiple policies. As a result, we obtain a better overlap in terms of the number of user-story interactions under the evaluated counterfactual policies..


\subsection{Analytical framework}

We start by enriching the analytical framework presented in Section \ref{sectionoffline}. In particular, we model the number of interactions in a period, the role of the position in the slate of stories, present the targeted estimand, and the proposed estimator.

Consider a period $D$ in which users interact with $n_{i}(D)$ stories; $n_{i}(D)$ is a random variable drawn from distribution $F_i(\cdot; D, \theta_{i})$. We make Assumption \ref{ass_1}.

\begin{assumption}\label{ass_1}
$n_i(D) \sim F_i(\cdot; D, \theta_{i})$, where $\theta_{i}$ is a random variable independent across users.
\end{assumption}

Assumption \ref{ass_1} implies that the number of stories a user interacts with is independent of the stories the user interacted with previously and the story interactions of other users. By Assumption \ref{ass_1} we also let users have types (e.g., heavy or light users) which determine how many stories they typically interact with. \footnote{Results presented in Section \ref{ATE_section}, indicate that Assumption \ref{ass_1} might not hold. Results from the randomized experiment show that the number of user-story interactions increases under the personalized policy. Therefore, the evaluation carried out under the assumption that there are no additional user-story interactions will render a conservative assessment of the gain in \emph{Total Story Engagement} .} Stories that a user $i$ interacts with in time period $D$ are indexed by $t_{i} \in \left\{1,2,...,n_{i}(D) \right\}$. Stories are placed in different ranks on a slate. Let $r \in \left\{1,...,15\right\}$ be ranks on the slate. 

Treatment is the assignment of a story $j$ on rank $r$ to a user $i$ in the $t_{i}$-th interaction. Treatment assignment is a random variable $w_{i,t_i} \in \mathcal{W} \equiv \left\{(1,1), (1, 2), .. (1, 15), .. (J, 1), ...,(J,15) \right\}$, where $J$ is the total number of stories, and 15 is the number of ranks on a slate. Treatment $W$ is a random variable with support in $\mathcal{W}$ and $W \sim W_{i}^{D}$, $w$ is a realization of $W$.  Let $E_{i, t_{i}}(w) \in \left\{0,1\right\}$ be the exposure outcome. $E_{i, t_{i}}(w)$ measures whether the story was exposed to the user - takes the value of one when the user has interacted with a story on the screen of the phone and zero otherwise. Let $U_{i,t_{i}(w)}$ be the potential engagement outcome. $U_{i,t_{i}(w)}$ measures the level of engagement of a user with the treatment (viewed, started, or completed the story).  $Y_{i, t_{i}}(w)$ be the potential outcome for user $i$  in interaction $t_{i}$ from the treatment $w$. Finally, the observed outcome depends on exposure and engagement:

\begin{align}
    Y_{i, t_{i}}(w) = \begin{cases} U_{i,t_{i}(w)} & \text{ if } E_{i, t_{i}}(w) = 1   \\ 
    NA & \text{ if }  E_{i, t_{i}}(w) = 0, \end{cases}
\end{align}
\ayush{proposal}
% \begin{align}
%     Y_{i, t_{i}}(w) = \begin{cases} U_{i,t_{i}(w)} & \text{ if } E_{i, t_{i}}(w) = 1   \\ 
%     NA & \text{ if }  E_{i, t_{i}}(w) = 0, \end{cases}
% \end{align}
$$
y_{it_i} = \sum_{j=1}^{J}\mathbb{1}(W_{it} = w)Y_{it_i}(w),
$$

where $NA$ means that the outcome of the treatment is that the engagement is not observed. We make Assumption \ref{ass_rank}.

\begin{assumption}\label{ass_rank}
Exposure outcome does not depend on the story but depends on the rank on the slate
\[
E_{i,t_{i}}(w) \indep j \text{ }\forall{j}  .
\]

Engagement outcomes of a user story interaction are independent of story rank in a slate
\[
U_{i,t_{i}}(w) \indep r \text{ }\forall{r}  .
\]

Additionally, we assume that for any user, the order of stories in the period does not impact outcomes
 \[
 Y_{i,k_{i}}(j) = Y_{i,l_{i}}(j),
 \]
 for all $i$, $k_{i}$ and $l_{i}$.

\end{assumption}

In \emph{Freadom}, users must manually scroll to the right before they see a new story card, and once they are looking at the story, they do not see other stories. For these reasons, we believe that Assumption \ref{ass_rank} well approximates users' behavior. By Assumption \ref{ass_rank} a story's order in the period does not impact potential outcomes, thus, we simplify notation, we write $Y_{it_{i}}(j)$ as $Y_{it}(j)$. 











Users and stories are characterized by unobserved characteristics. Let $x^u_i$ be a realisation of random variable $X^u$ which has support in $\mathcal{V}_x^u$, i.e., users are characterized by true unobserved random vectors $x^{u_1}, x^{u_2}, .. , x^{u_I}$; here the superscript $u$ indicates that these vectors are unobserved. Similarly, for stories, $z^u_j$ is a realization of random variable $Z^u$ which has support in $\mathcal{V}_z^u$. Thus, stories are characterized by true unobserved random vectors $z^{u_1}, z^{u_2}, .. , z^{u_J}$. Here, the superscript $u$ indicates these vectors are unobserved. We make Assumption \ref{unconf}.

\begin{assumption}\label{unconf}
Potential outcomes conditioned on user and story characteristics are independent across users and stories 
\[
Y_{it}(l) \perp Y_{i't}(k)|x_{i}^{u} , x_{i'}^{u}, z_{j}^{u} , z_{k}^{u}, 
\]
for all $i,i'$ and for all $l,k$.
\end{assumption}

Finally, we denote the observed outcome from a user-story interaction as 

$$
y_{it} = \sum_{j=1}^{J}\mathbb{1}(W_{it} = w)Y_{it}(j).
$$

\paragraph{Recommendation policies.} A recommendation policy is a mapping from user covariates to treatment assignment probabilities:

$$
\pi: \mathcal{V}_{x} \longrightarrow \mathcal{W} .
$$

The value of the policy depends on outcomes of user-story interactions. We define the value of the policy for a user $i$ as

\begin{align}\label{policy_value}
Q_i(\pi) = \sum_{t=1}^{n_i(D)}\mathbb{E}_{w \sim \pi(X_i)}\left[Y_{it}(w)\right].
\end{align}

The total value of a policy is the sum of values of individual users
$$
Q(\pi;D) = \sum_{i \in N_{D_{J}}} Q_i{(\pi)},
$$

 where $N_{D_{J}}$ is the number of users in period $D$. By weighting the individual user-story interactions equally, we are effectively putting a higher weight on users that consume many stories. 

\subsection{Empirical approach for policy learning and evaluation}

Policy learning and policy evaluation are carried out in separate time periods. We denote the policy learning period as $D^{1}$ and policy evaluation as $D^{2}$. In each period, we observe data $L_{D} \equiv (U_{i}, Z_{i}, O_{i})$, which summarizes active users, stories shown to those users, and the outcomes of user-story interactions.

We learn two types of recommendation policies: a popularity-based policy, using a two-way fixed effects model, and a personalized policy, using matrix factorization. Let the $\Pi$ denote the space of policies

\[
\pi^{M}(D^{1}) = \left\{M(D^{1}): \pi \in \Pi \right\},
\]
where $M(D^{1})$ is a Machine Learning algorithm (in our case, either two way fixed effects or matrix factorization), using which we learn a policy given a dataset $D^{1}$. Such a model is trained on a training set, evaluated on a test set, and tuned on a validation set, where the training, test and validation sets are random splits of the full dataset $D^{1}$. We perform hyperparameter tuning, which trains the model on the training set selects the model with the best performance on the validation set.

To evaluate the policy $\pi^{M}(D^{1})$, we employ the doubly robust estimator of $Q(\pi;D^{2})$ \citep{gilotte2018offline} \citep{zhou2022offline}. The estimator is shown in Equation \ref{off_estimator}.

\begin{align}\label{off_estimator}
\hat{Q}\left(\pi; D^{2}, \hat{e}^\pi, \hat{e}^T, \hat{y}(x_{i}, z_{j})\right) = \frac{1}{n_{D^{2}}} \sum_{(i, j, t_i, y_{it}) \in D^{2}}\left[\frac{\hat{e}_{it}(x_{i}, z_{j})^\pi}{\hat{e}_{it}(x_{i}, z_{j})^T} * (y_{it} - \hat{y}_{it}(x_{i}, z_{j})) + \mathbb{E}_{\pi_T}[\hat{y}_{it}(x_{i}, z_{j})] \right],
\end{align}

where $n_D^{2}$ is the number of user-story interactions in period $D^{2}$, $\hat{y}_{it}(x_{i}, z_{i})$ is an estimate of the story engagement for interaction $t$ for user $i$, and estimated representations of user and story characteristics $x_{i}, z_{i}$; $\hat{e}_{ijt}^T$ is an estimate of the propensity of treatment under the data collection policy $T$, and $\hat{e}_{ijt}^\pi$ an estimate of the propensity of treatment under the policy $\pi$.


To compute $\hat{y}_{it}(x_{i}, z_{i})$, we first estimate $x_{i}$ and $z_{i}$ using learned representations from matrix factorization of user-story interactions in period $D^{2}$, as well as use observed characteristics of users and stories. Finally, we predict $\hat{y}_{it}(x_{i}, z_{i})$ using a Regression Forest.

For a doubly robust off-policy estimate, we use two treatment propensities: first, $\hat{e}^{T}_{itj}(x_{i}, z_{j})$ propensity of a user $i$ interacting with story $j$ under policy $T$ the data-generating policy and second, $\hat{e}^{\pi}_{itj}(x_{i}, z_{j})$ the treatment propensity under the evaluated policy $\pi$.

In practice, we consider the following propensity models; Let $\hat{e}_{pers}$ be an estimate of the propensity model under the personalized policy. We know these propensities because they are a part of the recommendation system we designed. Let $\hat{e}_{pop}$ be an estimate of the propensity model under the popularity policy. Similar to the $\hat{e}_{pers}$, we know this as we construct this recommendation policy as well, using our Two Way Fixed Effects comparison model. Both $\hat{e}_{pers}$ and $\hat{e}_{pop}$ are distributions over the \textit{top K, K=15} stories under the respective algorithm, where the distribution is given by observed position effects, which we estimate from data.\footnote{We are able to estimate approximate position effects as recommendations are served from an editorial policy prior to the experiment.} Let $\hat{e}_{edit}$ be an estimate of the propensity model under the editorial-based policy. We estimate this policy using log data as a simple mean exposure probability per story per grade level, not personalized to a user; we know that this is how editorial recommendations were given out, as communicated to us by \emph{S2M}.

We summarize the algorithm for policy learning and evaluation in Algorithm \ref{alg:off_policy}.

\begin{algorithm}
\caption{Doubly Robust Off Policy Evaluation}\label{alg:off_policy}
\begin{algorithmic}
    \State {\bfseries Input:} Data $L_{D} \equiv (U_{i}, Z_{i}, O_{i})$, i.e. (user, story, story engagement) tuples, consisting of $n$ logs, User Representations $\mathcal{X}$, Story Representations $\mathcal{Z}$, true data collection propensity model $\hat{e}^{T}$, target policy $\hat{e}^{\pi}$
    \State {\bfseries Result:} Off Policy Estimate $\hat{Q}(\pi)$ under the target policy
  \end{algorithmic}

  \begin{algorithmic}[1]
  \State $\mu = \text{RegressionForestModel}(L_D, \mathcal{X}, \mathcal{Y})$
  \ForEach {log $(X_i, Z_i, O_i) \in L_D$ }
    \State $\hat{y}_i = \mu(X_i, Z_i)$
    \State $\hat{w}_i = \frac{\hat{e}^{\pi}(X_{i}, Z_{i})}{\hat{e}^{T}(X_{i}, Z_{i})}$
  \EndFor
  \State $\hat\mu_{\pi} = \frac{1}{n}\Sigma_{(X_{i}, Z_{i}, O_{i}) \in L_{D}}\hat{e}^{\pi}(X_{i}, Z_{i})*\hat{y}_{i}$
  \State $\hat{Q}(\pi) = \frac{\Sigma_{i \in 1..n} w_{i} \hat{y}_{i}}{\Sigma_{i \in 1..n} w_{i}} - \hat\mu$
  \State \Return $\hat{Q}(\pi)$
  \end{algorithmic}
\end{algorithm}




\subsection{Empirical Results}

We consider three policies: $\pi_{pers}$ - the personalized recommendation system, $\pi_{pop}$ - the popularity policy based on a two-way fixed effects model, and  $\pi_{edit}$, which is the baseline editorial policy. We use five different data samples in this analysis: 

\begin{itemize}
    \item $D_{pre}$ : data from the period before the randomized experiment described in Section 4 (July 22, 2020 - July 21, 2021). In this sample all data is generated under $\pi_{edit}$, the editorial system.
    \item $D_{exp}$ : data from the experimental period (July 22, 2021 - August 4, 2021). In this sample there are two policies deployed: users in the treatment group using the \emph{Recommended Story} tray receive stories from $\pi_{pers}$, a personalized policy, while users in the control group get content recommendations in the \emph{Recommended Story} tray from $\pi_{edit}$. In all other trays in the app, data is generated from $\pi_{edit}$.
    \item $D_{post1}$ : data from the period right after the experiment (August 5, 2021 - August 18, 2021). In this sample, all users get personalized recommendations in the \emph{Recommended Story} tray and in all other trays from $\pi_{edit}$.
    \item $D_{post2}$ : data from a longer period after the experiment (August 19, 2021 - March 2, 2022). In this sample, all users get personalized recommendations in the \emph{Recommended Story} tray and in all other trays from $\pi_{edit}$.
    \item $D_{post3}$ : data from a period after $D_{post2}$ (March 3, 2022 - March 16, 2022). In this sample, all users get personalized recommendations in the \emph{Recommended Story} tray and in all other trays from $\pi_{edit}$.
\end{itemize}

We, first, use $D_{pre}$ to learn $\pi_{pers}$ and evaluate it in $D_{exp}$; this analysis aims to compare off-policy estimates with the estimates from a randomized experiment. Second, we exploit the fact that $D_{post2}$ is a longer period with more observations (more users have been active in this period) to learn $\pi_{pers}$ and $\pi_{pop}$ and evaluate them in $D_{post3}$; this analysis is aimed at comparing engagement under the popularity-based and personalized policies.   Third, we use $D_{exp}$ to learn two popularity-based policies, one from the data generated using $\pi_{pers}$, i.e. from users in the treatment group, and the other using $\pi_{edit}$, i.e. from users in the control group; this analysis aims to investigate if the personalized model does better simply because it discovers more popular stories, or because it indeed personalizes well, compared to the baseline editorial policy. We evaluate these policies in $D_{post1}$. Figure \ref{fig:timeline} visualizes this workflow.


    	\begin{figure}[H]
    	\caption{Data samples used for off-policy evaluation.}
			\centering
			\includegraphics[scale=0.6]{images/timeline.PNG}
			\label{fig:timeline}
		\end{figure}
		
	
Policies depend on the sample used. We add superscripts to policies to distinguish which data period was used in policy learning, e.g.,  $\pi_{pop}^{D_{pre}}$ is the popularity-based policy trained on data from the pre-experimental period: $D_{pre}$. 
 


\subsubsection*{Estimates of gains from the personalized policy using off-policy evaluation versus the randomized experiment.}

Let $\hat{Q}_{RCT}(\pi_{pers})$ be an estimate of the policy value from Equation \ref{policy_value} using the OLS estimator based on the randomized experiment discussed in Section 4 and $\hat{Q}(\pi_{pers})$  be the estimate from the off-policy estimator in Equation \ref{off_estimator}. In Section \ref{off_problems}, we argued that assuming additive separability of user-item interactions is required for the off-policy estimator to be consistent. Now we compare the estimate from the randomized experiment to the off-policy estimate and check whether we would obtain similar findings using off-policy evaluation and the randomized experiment. Thus, we are interested in testing whether $H0: \hat{Q}_{RCT}(\pi_{pers}) - \hat{Q}(\pi_{edit}) = \hat{Q}(\pi_{pers}) - \hat{Q}(\pi_{edit})$. \footnote{It would also have been useful to compare the popularity based policy to the personalized and editorial policies in the same way, but we were unable to do this from the experimental period data due to insufficient overlap} To construct the off-policy estimator, we use the same policy as deployed in the experiment (that is, a policy learned in $D_{pre}$). Both policies are evaluated in $D_{exp}$. Figure \ref{fig:off1} presents the results.

    	\begin{figure}[H]
    	\caption{Policy value estimates from off-policy estimator and the randomized experiment}
			\centering
			\includegraphics[scale=0.5]{images/off_policy_barplot1.png}
			\label{fig:off1}
						\caption*{\footnotesize{\textit{Note: Comparison of estimates of the value of the introduction of the  personalized policy using the off-policy estimator and the OLS estimator based on the experiment. In blue is the OLS estimate of $\hat{Q}_{RCT}(\pi_{pers}) - \hat{Q}(\pi_{edit})$ using the randomized experiment. We adjust for the rank in the tray in which the story was displayed and for the past utilization. Standard errors are clustered at a user level. We consider all users. In red, we present estimates using the off-policy estimator: $\hat{Q}(\pi_{pers}) - \hat{Q}(\pi_{edit})$. On the left, we show the estimate across all users, then for heavy \emph{Story Engagement} users, and finally for light \emph{Story Engagement} users. Whiskers show confidence intervals. }}}
		\end{figure}

		
We find that  we cannot reject that the difference between the OLS and off-policy estimates is statistically insignificant.  We additionally present the off-policy estimates of the gains due to personalization for heavy and light users. We find that the point estimate is higher for heavy users than for light users, which is consistent with the findings in the randomized experiment, but the difference is statistically insignificant. 

\subsubsection*{Off-policy comparison of the values of personalized and popularity-based policies}

To justify investments in a personalized policy, we want to show that similar gains cannot be achieved through a simpler popularity-based policy. To do that, we learn $\pi_{pers}$ and $\pi_{pop}$, estimate their values, and compare them to the value from $\pi_{edit}$. For this task, we use $D_{post2}$ to learn the policies, which is a period of over six months in which both algorithms have been deployed. By doing so, we have more observations and better story overlap than in the experimental period. We use $D_{post3}$ to evaluate the policies. We want to test the following hypotheses:

\begin{align*}
H0^{A}_{1} : Q(\pi_{pers}) =  Q(\pi_{edit}), \\
H0^{A}_{2} :Q(\pi_{pop}) =  Q(\pi_{edit}), \\
H0^{A}_{3} :Q(\pi_{pop}) =  Q(\pi_{pers}).
\end{align*}

Additionally, we evaluate policies for heavy and light users.


\begin{align*}
H0^{A}_{4} : Q(\pi_{pers}|G_{i} = g) =  Q(\pi_{edit}|G_{i} = g), \\
H0^{A}_{5} :Q(\pi_{pop}|G_{i} = g) =  Q(\pi_{edit}|G_{i} = g), \\
H0^{A}_{6} :Q(\pi_{pop}|G_{i} = g) =  Q(\pi_{pers}|G_{i} = g),
\end{align*}
where $g \in \left\{ low, high\right\}$ represents whether the user $i$ is a high engagement (in the top 50th percentile of the pre-experimental \emph{Story Engagement}) or a low engagement user.  Figure \ref{fig:off2} shows the results.

    	\begin{figure}[H]
    	\caption{Off-policy comparison of policy value estimates}
			\centering
			\includegraphics[scale=0.6]{images/off_policy_barpot2.png}
			\label{fig:off2}
						\caption*{\footnotesize{\textit{Note: Comparison of estimates of the value of $\pi_{pers}$, $\pi_{pop}$ and $\pi_{pop}$. Height of each bar corresponds to $\hat{Q}(\pi_{policy A}) -\hat{Q}(\pi_{policy B})$. Red bars compare personalized and editorial policies, green ones personalized and popularity policies, and blue ones popularity and editorial policies. On the left, we present results for all users, in the middle for heavy users, and on the right for light users. Whiskers show confidence intervals. }}}
		\end{figure}
		
First, we estimate that the value of the personalized policy is higher than that of the editorial policy for both heavy and light users. Second, we estimate that the popularity-based policy has a higher value than the editorial policy for heavy users. Finally, comparing the personalized and popularity-based policies, we estimate that all user groups are better off under the personalized policy.\footnote{We note that these results conform with the results from off-policy evaluation during the experiment period, but since we have more data, they give us more precise estimates and have higher magnitudes. We are likely seeing higher magnitudes in the post-period since, due to more data, we are able to learn better-personalized policies, which is a known property of matrix factorization.}
		

\subsubsection*{Are the gains in the personalized policy due to better popular stories or due to personalization?}
 The outcome model used for the personalized recommendation system has two components: user and item fixed effects and the interaction of user and story latent features. This means that the gains due to the new recommendation system can come from a better selection of popular stories than under the editorial system and from the personalization of content assignment. 
 
In carrying out the randomized experiment, user interaction data was collected under both the editorial and the personalized policies simulaneously.  We exploit this fact, to learn popularity-based models from each experimental arm (i.e., models are trained on the $D_{exp}$ sample). We report the off-policy estimates of these policies on post-experimental data right after the experiment ($D_{post1}$). We denote $\pi_{pop}^{D_{C}}$ as the popularity-based model trained on data generated under $\pi_{edit}$ , and denote $\pi_{pop}^{D_{T}}$ as the popularity-based model trained on data generated under $\pi_{exp}$. The comparison of these two popularity-based policies also allows us to analyze whether the story exploration under the two models leads to differences in the success rate of discovering highly popular stories. We are testing the following hypotheses: $H0^{1}: \hat{Q}(\pi_{pop}^{D_{C}}) = \hat{Q}(\pi_{edit})$ and $H0^{2}: \hat{Q}(\pi_{pop}^{D_{T}}) = \hat{Q}(\pi_{edit})$. Figure \ref{fig:off3} shows the results.


    	\begin{figure}[H]
    	\caption{Off-policy comparison of policy value estimates}
			\centering
			\includegraphics[scale=0.6]{images/off_policy_barplot3.png}
			\label{fig:off3}
						\caption*{\footnotesize{\textit{Note: Comparison of estimates of the value of $\pi_{pop}^{D_{exp,C}}$, $\pi_{pop}^{D_{exp,T}}$ and $\pi_{edit}$. Height of each bar corresponds to $\hat{Q}(\pi_{policy A}) -\hat{Q}(\pi_{policy B})$. In red bars, we show $Q(\pi_{pop}^{D_{exp,C}}) -Q(\pi_{edit})$ and in blue bars $Q(\pi_{pop}^{D_{exp,T}}) -Q(\pi_{edit})$. On the left, we consider all users of the app; in the middle, we focus on heavy users, and on the right, on the light users. Whiskers show confidence intervals. }}}
		\end{figure}
		
		
First, we estimate that both popularity-based policies have a higher value than the value under the editorial policy. Second, comparing the two popularity-based policies, we find they create similar value for heavy users. The popularity-based policy trained from the data generated from the personalized recommendations has a higher estimated value for light users than the popularity-based policy trained on the editorial-system data.

Evidence presented in Figure \ref{fig:off3} suggests the editorial and personalized systems are similarly effective in terms of discovering popular stories. Hence, we conclude that the gains in the personalized policy are due to personalization and not only due to a better selection of popular stories.


